Design and Characterization of a Balloon-Borne Diffraction-Limited Submillimeter Telescope Platform for BLAST-TNG

The Next Generation Balloon-borne Large Aperture Submillimeter Telescope (BLAST-TNG) is a submillimeter mapping experiment planned for a 28 day long-duration balloon (LDB) flight from McMurdo Station, Antarctica during the 2018-2019 season. BLAST-TNG will detect submillimeter polarized interstellar dust emission, tracing magnetic fields in galactic molecular clouds. BLAST-TNG will be the first polarimeter with the sensitivity and resolution to probe the $\sim$0.1 parsec-scale features that are critical to understanding the origin of structures in the interstellar medium. With three detector arrays operating at 250, 350, and 500 $\mu$m (1200, 857, and 600 GHz), BLAST-TNG will obtain diffraction-limited resolution at each waveband of 30, 41, and 59 arcseconds respectively. To achieve the submillimeter resolution necessary for its science goals, the BLAST-TNG telescope features a 2.5 m aperture carbon fiber composite primary mirror, one of the largest mirrors flown on a balloon platform. Successful performance of such a large telescope on a balloon-borne platform requires stiff, lightweight optical components and mounting structures. Through a combination of optical metrology and finite element modeling of thermal and mechanical stresses on both the telescope optics and mounting structures, we expect diffraction-limited resolution at all our wavebands. We expect pointing errors due to deformation of the telescope mount to be negligible. We have developed a detailed thermal model of the sun shielding, gondola, and optical components to optimize our observing strategy and increase the stability of the telescope over the flight. We present preflight characterization of the telescope and its platform.

==> Alighnment.tex <==
\section{Telescope Alignment and Integration}

The telescope has been completed. It will be installed on the gondola during the payload integration at the NASA/CSBF facility in Palestine, TX in the summer of 2018. 

We'll use the laser tracker to align the telescope by surveying permanently installed retroreflectors.

Additional focusing tests include de-focusing the secondary mirror to view an object in the telescope near field.

During flight, the telescope is focused by making beam maps of bright submillimeter point sources. This is repeated regularly throughout the flight. In between refocusing, the secondary mirror is automatically refocused based on a thermal model of the telescope mirrors and support structures, and the measured temperatures of each of these components. 

==> ScienceGoals.tex <==
\section{Science Goals}
\label{section:science}

The primary science goal of BLAST-TNG is to map the polarized thermal emission from galactic interstellar dust around star-forming regions and in the diffuse interstellar medium (ISM).
\begin{enumerate}

 \item{What role do magnetic fields play in star formation? What forces shape the molecular clouds which are the birthplace of stars in the ISM?}
 
 \item{What are the properties of interstellar dust? What can we learn about its composition from its spectral properties of its thermal and polarized emission?}

\end{enumerate}
